Caching Structures for Distributed Data Management in P2P-based Social Networks

Distributed applications require novel solutions to tackle problems that arise due to the scarcity of resources such as bandwidth, memory and processing power. One of these challenges is seen in distributed data management. The challenge is the two part problem of ensuring that the content is valid when accessed and updating it immediately when changed. This is especially difficult when considering p2p-based distributed online social networks, which aim to build reliable, secure social networking platforms on top of often unreliable and unsecure devices. In this paper, we propose three selection strategies, random, trend and social score, for a social caching mechanism. They consider the social interaction patterns in the social network. We implement and evaluate them in a DHT-based distributed online social networks called LibreSocial and show that the social score is the best strategy. Further we implement the social caching solution and also show that when used in combination with the existing caching solution almost all requests can be serviced via cache while retaining the consistency of data during updates.

==> IEEE-format-latex <==
#!/usr/bin/perl -w
#
# fmtlatex - put a LaTeX document into a canonical formatting suitable
# for comparing genuine differences rather than just formatting
# differences
# 
# Copyright (C) 2007   Andrew Stacey <stacey@math.ntnu.no>
# 
# This program is free software; you can redistribute it and/or mod
# ify it under the terms of the GNU General Public License as
# published by the Free Software Foundation; either version 2 of the
# License, or any later version.
# 
# This program is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
# General Public License for more details.
# 
# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 59 Temple Place - Suite 330, Boston, MA 02111-1307,
# USA.
# 

use strict;
use Getopt::Long qw(:config auto_help bundling);
use Pod::Usage;

my (
    $shortmath,
    $shortarray,
    $indent,
    $parsep,
    $state,
    $descend,
    $ascend,
    $previous,
    $preamble,
    $dopreamble,
    $curindent,
    $man,
    $help,
    $gpl,
    $version,
    $verstring
    );

$verstring = "fmtlatex version 1.1, Copyright (C) 2007--2013 Andrew Stacey\nfmtlatex comes with ABSOLUTELY NO WARRANTY; for details type\n `fmtlatex --man'.\nThis is free software, and you are welcome to redistribute it under certain\nconditions; type `fmtlatex --man' for details.";

# Default options

# How long should inline maths be before it gets its own line?
$shortmath = 20;

# Ditto for array-like environments
$shortarray = 40;

# Do we want indentation?
$indent = " ";

# Commandline options

GetOptions (
    "p|preamble" => \$dopreamble,
    "i|indent=i" => sub {my ($a, $b) = @_; $indent = $indent x $b;},
    "m|math=i" => \$shortmath,
    "a|array=i" => \$shortarray,
    "man" => \$man,
    "h|?|help" => \$help,
    "gpl" => \$gpl,
    "V|version" => \$version
    ) or pod2usage(2);

die "$verstring\n" if $version;
pod2usage(-exitval => 1, -verbose => 1) if $help;
pod2usage(-verbose => 2 ) if $man;
exec 'perldoc perlgpl' if $gpl;


# Regular expression to match a lines that start or separate
# paragraphs.  Copied from Emacs, had to translate \> to \b and $$
# seemed in the wrong place (needed preceeding backslash in Emacs
# version).


# If the start of the line matches something here then it is not part
# of the previous paragraph.

$parsep = '^ (?: \f |
                    \s* (?: $        |
                            %        |
                            \$\$     |
                            \\\\[][] |
                            \\\\ (?: b(?:egin   | ibitem)            |
                                     c(?:aption | hapter)            |
                                     end                             |
                                     footnote                        |
                                     item                            |
                                     label                           |
                                     marginpar                       |
                                     n(?:ew(?:lin | pag)e | oindent) |
                                     par(?:agraph | box | t)         |
                                     s(?:ection |
                                         ub(?:paragraph |
                                              s(?:(?:ubs)?section)
                                           )
                                      )                              |
                                     [a-z]*(page | s(?:kip | space))
                                 ) \b
                        )
                )';

# Certain commands should be on their own line.  The following regexp
# determines which.  Note, we only add an eol after them if they
# (essentially) _begin_ the current line.

$state = '^ \s* (?: \$\$   |
                        \\\\[][] |
                        \\\\ (?: b(?:egin   | ibitem)            |
                                 c(?:aption | hapter)            |
                                 end                             |
                                 footnote                        |
                                 item                            |
                                 label                           |
                                 marginpar                       |
                                 n(?:ew(?:lin | pag)e | oindent) |
                                 par(?:agraph | box | t)         |
                                 s(?:ection |
                                     ub(?:paragraph |
                                          s(?:(?:ubs)?section)
                                       )
                                  )                              |
                                 [a-z]*(page | s(?:kip | space))
                              ) \b
                      )';


# Regular expression to match a descent or ascent of depth

$descend = ' \\\\ \[       |
                \\\\ begin \b |
                \{ ';

$ascend =  ' \\\\ \]     |
                \\\\ end \b |
                \}';

# Actually, we work on the previous line
$previous = "";

# And we start with no indentation
$curindent = 0;

while (<>) {
    # Skip between '\documentclass' and '\begin{document}'

    if (/^[^%]*\\documentclass\b/) {
	if ($previous) {
	    &output($previous);
	    $previous = "";
	}
	$preamble = 1;
    }

    if (s/^([^%]*\\begin\{document\})\s*//) {
	$dopreamble or $preamble and print $1 . "\n";
	$preamble = 0;
    }

    $dopreamble or $preamble and print and next;

    # Do we remove the eol from the previous line?  Check the current
    # line against the paragraph separator and remove the eol if it
    # doesn't match.

    if (!/$parsep/x
	and ($previous !~ /%/)
	and ($previous !~ /^\s*$/)) {
	# This line appears to be in the same paragraph as the
	# previous one, so we ought to chomp the previous one.  There
	# are two cases where we don't: if the previous line was
	# (essentially) blank then we don't chomp it, and if the
	# previous line ended in a comment then we don't.  If we do
	# chomp, we add a whitespace to ensure that the whitespace
	# count is not effected.
	if ($previous =~ s/[\r\n]+$//) {
	    $previous .=  " ";
	}
    }
    # does $previous have an eol?

    if ($previous =~ /\n/) {
	&output($previous);
	$previous = "";
    }
    $previous .= $_;
}

&output($previous);

exit 0;

sub output {
    my ($line) = @_;
    my $comment = "";
    $line =~ s/[\r\n]+$//;


    $line =~ s/(?:^|(?<=[^\\]))(%.*)// and $comment = $1;

    # So much for removing eols, do we want to add any in?

    # Rule 1.  New sentence, new line.  Use TeX's algorithm: .!? end a
    # sentence unless . is preceeded by a capital letter.

    $line =~ s/([^A-Z]\.|^\.|\?|!) +/$1\n/g;

    # Rule 3.  Long inline maths is on its own line.

    # Break on starting maths:
    #
    # Must have a whitespace to break on, and don't break if the break
    # point is already at the start

    $line =~ s/([^\n\s])[\n\s]+(\S*(?:\\\(|\$))/$1\n$2/g;

    # If the closing delimeter occurs less than $shortmath from the
    # start, remove the break; otherwise add an ending break.
	    
    $line =~ s/(^\S*(?:\\\(|\$).{$shortmath,}\\\)\S*) */$1\n/mg;
    $line =~ s/\n(\S*(?:\\\(|\$).{0,$shortmath}\\\)\S*)/ $1/g;

    # Rule 4.  Tables and arrays are split according to lines, and
    # entries if long enough.  Ought to make this the same throughout
    # the table but that involves remembering too much information.

    # Break after & and \\'s.
    # We want to ensure that we don't _add_ any whitespace here so if there
    # wasn't any originally we add a comment string before the eol.  Also,
    # don't break if we are already (effectively) broken.

    $line =~ s/(\&|\\\\)\s+(?!%|$)/$1\n/g;
    $line =~ s/(\&|\\\\)(?!\s|%|$)/$1%\n/g;

    # If two adjacent column entries are shorter than the given
    # minimum length, remove the eol between them.  Can't just add 'g'
    # modifier to the regexp as we may need to join several entries
    # together and so need to backtrack.

    while ($line =~ s/(^.{0,$shortarray}\&)\n(.{0,$shortarray}(?:\&|\\\\|\n))/$1 $2/s) {};

    # Rule 2.  Change-of-states that occur at the start of a line get their
    # own line.  Need to include any arguments on that line.

    my $newline = "";
    while ($line =~ s/($state)//x) {
	$newline .= $1;
	my $nextarg;
	($nextarg, $line) = &nextarg($line);
	while ($nextarg !~ /^ *$/) {
	    $newline .= $nextarg;
	    ($nextarg, $line) = &nextarg($line);
	}
	$newline .= "\n";
    }
    $line = $newline . $line;
    # Make sure we haven't inadvertantly _added_ a double eol or any
    # excessive whitespace

    $line =~ s/\n+/\n/g;
    $line =~ s/^ +//mg;
    $line =~ s/  +/ /g;

    # Add some basic contextual indentation.

    if ($indent) {
	my @lines = split("\n", $line);
	for (my $i = 0; $i <= $#lines; $i++) {
# If the line _starts_ with an ascender or an \item, cancel an indent
	    my $offset = ($lines[$i] =~ /^(?:$ascend|\\item)/x ? -1 : 0);
# If the line _starts_ with inline maths, add an indent.  Note this and the
# previous can't _both_ match so we're okay setting $offset to 1 if this
# matches.
	    $offset = ($lines[$i] =~ /^\s*\\\(/ ? 1 : $offset);
	    $lines[$i] = $indent x ($curindent + $offset) . $lines[$i];

# Count the ascenders and descenders in the line to get the current
# indent for the next line.
# Actually work on a 'decommentised' version of the line so that stuff in
# comments doesn't effect the count.
	    my $decomment = $lines[$i];
	    $decomment =~ s/%.*//;
	    while ($decomment =~ /$descend/gx) {
		$curindent++;
	    }
	    while ($decomment =~ /$ascend/gx) {
		$curindent--;
	    }
	}
	$line = join("\n", @lines) . "\n";
    }

# Finally, don't indent comments

    $line =~ s/^ +%/%/;

    $line =~ s/[\r\n]+$//;
    print $line . $comment . "\n";
}


# Extract the next block from the string
sub nextarg {
    my ($string) = @_;
    my $first = "";

# Bail out if we didn't actually get anything
    return ("", "") unless ($string);

    if ($string =~ s/^(\{.*?\})//s) {
# We need to ensure that the braces are balanced.
	$first = $1;
	my $c = ($first =~ tr/{/{/) - ($first =~ tr/}/}/);
	while ($c > 0 && $string =~ /}/) {
	    $string =~ s/^(.*?})//s;
	    $first .= $1;
# Count the number of opening and closing braces in $first
	    $c = ($first =~ tr/{/{/) - ($first =~ tr/}/}/);
	}
	return ($first, $string);
    }

    if ($string =~ s/^(\[.*?\])//s) {
# We need to ensure that the curly braces are balanced.
	$first = $1;
	my $c = ($first =~ tr/{/{/) - ($first =~ tr/}/}/);
	while ($c > 0 && $string =~ /\]/) {
	    $string =~ s/^(.*?])//s;
	    $first .= $1;
# Count the number of opening and closing braces in $first
	    $c = ($first =~ tr/{/{/) - ($first =~ tr/}/}/);
	}
	return ($first, $string);
    }
# All else, just return first character

    $string =~ s/(.)//s;

    return ($1, $string);
}

__END__

=head1 NAME

fmtlatex - format a LaTeX document putting it into a canonical format suitable for finding genuine differences rather than formatting differences

=head1 SYNPOSIS

 fmtlatex [OPTIONS] [FILES]

Format [FILES] or standard input according to the rules, modified by [OPTIONS] if specified, sending output to standard output.

Example: fmtlatex < paper.tex > paper.fmt.tex

 Options:
  -p, --preamble    process the preamble
  -m, --math NUM    inline math longer than NUM gets its own line
                    (default: 20)
  -a, --array NUM   array-like entries longer than NUM get their own line
                    (default: 40)
  -i, --indent NUM  add indentation using NUM multiples of " "
                    (default: 1)
  --man             print man page
  -h,-?, --help     print basic help
  -V, --version     print version information
  -gpl              print GPL

=head1 DESCRIPTION

B<fmtlatex> formats a LaTeX document into a standardised layout according to the following rules:

=item B<1.> Each sentence is on its own line.

=item B<2.> Change-of-state commands are on their own line (e.g. \begin or \[)

=item B<3.> Long pieces of inline maths are on their own line

=item B<4.> Long array entries are on their own line, otherwise array rows are on their own line.

The other guiding principle is that the original author is assumed to be intelligent.

B<fmtlatex> works by going through a LaTeX document, supplied either on the command line or via standard input, line by line and removing or adding end-of-line characters according to the above rules.  The purpose is to produce a document in a standardised form that can be compared with a previous version using, say, I<diff> so that the differences shown are due to actual differences of content and not accidental differences of formatting.

Minor modification of the algorithm can be done by changing the values of certain options.  Major modification can be done by hacking the program.

=head1 OPTIONS

=over 8

=item B<-p, --preamble>

Determines whether or not to process the preamble.  The default is to skip the preamble (everything between C<documentclass> and C<begin{document}>).

=item B<-m NUM, --math NUM>

Designates how long a stretch of inline maths has to be before it qualifies for its own line.  Note: the length is of the maths but there may be extra junk on the line as the program only inserts eols at existing whitespace.

Default: 20

=item B<-a NUM, --array NUM>

Designates how long an array entry has to be before it qualifies for its own line.  Note: both the current and next array entries have to be shorter than this to qualify for a single line.

Default: 40

=item B<-i NUM, --indent NUM>

The program also inserts basic indentation according to how "deep" the start of the current line is (it counts the number of '\\begin's, '\['s, and '{'s and their corresponding terminators) and indents accordingly.  NUM designates how many spaces corresponds to one indentation.

=item B<--man>

Display full man page.

=item B<-h, -?, --help>

Display basic help page.

=item B<-V, --version>

Display version information.

=item B<--gpl>

Display GPL.

=head1 NOTES

The indentation and inline math algorithms ignore '$' but the paragraph separation knows about them.  Basically, you shouldn't be using '$'s in a LaTeX document.  Coding for things like C<$a=b$$c=d$> is a hassle and I'd rather not bother if I didn't have to.

This program shouldn't introduce any TeXtual changes into your document.  A simple way to test this (before you delete the original), is to C<latex> the original and the formatted version each a few times, then C<dvips> them, and C<diff> the resulting postscript files.  You should see something like

 shell% diff original.ps new.ps
 3c3
 < %%Title: original.dvi
 ---
 > %%Title: new.dvi
 12c12
 < %DVIPSCommandLine: dvips original.dvi
 ---
 > %DVIPSCommandLine: dvips new.dvi
 14c14
 < %DVIPSSource:  TeX output 2007.12.20:1128
 ---
 > %DVIPSSource:  TeX output 2007.12.20:1159
 1560c1560
 < TeXDict begin 39139632 55387786 1000 600 600 (original.dvi)
 ---
 > TeXDict begin 39139632 55387786 1000 600 600 (new.dvi)

That is, no significant change at all.


=head1 BUGS

Whad'dya mean, "I've found a bug."?  Impossible.  There are no bugs,
only features.  To tell me about features, send an email to 

stacey@math.ntnu.no

With the following in the subject line:

Howay man, av fund ah borg een furmatleetach.

=head1 AUTHOR

Andrew Stacey

=head1 LICENSE

Copyright (C) 2007--2013   Andrew Stacey

This program is free software; you can redistribute it and/or mod ify
it under the terms of the GNU General Public License as published by
the Free Software Foundation; either version 2 of the License, or any
later version.

This program is distributed in the hope that it will be useful, but
WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU
General Public License for more details.

You should have received a copy of the GNU General Public License
along with this program; if not, write to the Free Software
Foundation, Inc., 59 Temple Place - Suite 330, Boston, MA 02111-1307,
USA.


